A Quadratically Enriched Correspondence Theorem

We quadratically enrich Mikhalkin's correspondence theorem. That is, we prove a correspondence between algebraic curves on a toric surface counted with Levine's quadratic enrichment of the Welschinger sign, and tropical curves counted with a quadratic enrichment of Mikhalkin's multiplicity for tropical curves.

==> temp.tex <==
In order to compute the quadratic weight of the parameterized rational curve~$C'$, we compute the product over all nodes of the curve of the determinant of the Hessian of a defining polynomial at every nodal point, up to squares. In order to compute the local contribution at every nodal point, we use the fact that this determinant can be compute up to squares directly from the parametrization.

Namely, let us assume that there are parameters~$t$ and~$s$ defining a non-degenerate double nodal point~$p$. The linear change of variable given by the tangent vectors $(x'(t),y'(t))$ and $ (x'(s),y'(s))$ of the parametrization at $p$, allows us to have an explicit local equation of the form~$\gamma u v+\mathrm{h.o.t.}$, where $\gamma\in k$ and $u,v$ are local coordinates. Therefore, minus the determinant of the Hessian of a defining equation at the node $p$ equals
\[\left(x'(t)y'(s)-x'(s)y'(t)\right)^{2},\]
up to squares in~$k$.
Hence, using the parametrization in \eqref{eq:parametrization}, we have that the local contribution at a node equals
\begin{equation}\label{eq:hesspar}
    \left[
\frac{mx(t)}{t} \frac{y(s)(qs-p)}{s(s-1)}-\frac{mx(s)}{s} \frac{y(t)(qt-p)}{t(t-1)}
\right]^2=\left(m(q-p)x(t)y(t)\right)^2\left[\frac{t-s}{t(t-1)s(s-1)}
\right]^2.
\end{equation}
Now, let us compute the coordinates of the nodes of~$C'$. The parameters $s$ and $t$ must satisfy the equations $(x(t),y(t))=(x(s),y(s))$ with $t\neq s$. Hence, we have that $s=t\mu$, where $\mu$ is a non-trivial $m$-th root of unity, and 
\[\frac{1-t}{1-\mu t}=\mu^{\frac{p}{q-p}}\nu,\]
where $\nu$ is a $(q-p)$-th root of unity. Put $\zeta=\mu^{\frac{p}{q-p}}\nu$.
Then, the parameters where there is a node are the solutions to the equations
\begin{equation}\label{eq:nodespar}
    t=\frac{1-\zeta}{1-\zeta\mu},\quad s=t\mu,\quad \zeta=\mu^{\frac{p}{q-p}}\nu,
\end{equation}
where $\mu^m=\nu^{q-p}=1$ and $\mu\neq1,\zeta\neq1,\zeta\mu\neq1$. Hence, the solutions are given by 
\begin{align} \label{eq:mupar}
    \mu=&\zeta_m^{i}     & i=1,2,\dots, m-1,\\ \label{eq:zetapar}
    \zeta=&\zeta_{m(q-p)}^{ip+jm} & ip+jm\not\equiv 0 \mod m(q-p),\\ \label{eq:zetamupar}
    \zeta\mu=&\zeta_{m(q-p)}^{iq+jm} &iq+jm\not\equiv 0 \mod m(q-p),
\end{align}
where $j=1,2,\dots, q-p$, and $\zeta_m$ and $\zeta_{m(q-p)}$ are primitive $m$-th and $m(q-p)$-th roots of unity, respectively. However, this counts twice the number of nodes since the branches of a node are unordered. 

Set $m_p=\frac{m}{d_p}$ and $m_q=\frac{m}{d_q}$. Let us remark that $ip+jm\equiv 0 \mod m(q-p)$ if and only if ${i\frac{p}{d_p}+jm_p\equiv 0} \mod m_p(q-p)$ and that if $i\frac{p}{d_p}+jm_p\equiv 0 \mod m_p(q-p)$, then~$i\frac{p}{d_p}\equiv 0 \mod m_p$. Since $\gcd(\frac{p}{d_p},m_p)=1$, we have that $i\equiv 0 \mod m_p$. So there are exactly~$d_p-1$ solutions to~$ip+jm\equiv 0 \mod m(q-p)$, namely when $i=m_pi'$, where~$i'=1,2,\dots,d_p-1$ and $j$ is the only solution to $j\equiv-i'\frac{p}{d_p}$ in range.
Analogously, there are $d_q-1$ solutions to~$iq+jm\equiv 0 \mod m(q-p)$, given by $i=m_qi'$, where~$i'=1,2,\dots,d_q-1$ and $j$ is the only solution to $j\equiv-i'\frac{q}{d_q}$ in range. Thus, there are $\frac{(m-1)(q-p)-(d_p+d_q-2)}{2}$ distinct nodes. By Pick's theorem, this correspond to~$\operatorname{Int}(\Delta')$ the number of interior lattice points in the triangle $\Delta'$.

Finally, we can compute the quadratic weight of the curve~$C'$ by multiplying  over the nodes of~$C'$ the expression in~\eqref{eq:hesspar}, or equivalently, by multiplying the square root of this expression over all solutions of~\eqref{eq:nodespar}, multiplying it by $-1$ for each node due to the fact that we interchange the roles of~$s$ and~$t$ in one of the instances of~\eqref{eq:nodespar} that describe the same node. Thus, the quadratic weight is the class of the quadratic form given by
\begin{equation}\label{eq:welnodes}
\displaystyle\prod_{\text{nodes of }C}\left[\frac{t-s}{t(t-1)s(s-1)}\right]^2=
(-1)^{\operatorname{Int}(\Delta')}\prod_{\mathrm{sols. to\eqref{eq:nodespar}}} \frac{t-s}{t(t-1)s(s-1)},
\end{equation}
since the product over the nodes of $C'$ of the factor $(x(t)y(t))^2$ is a square in~$k$.
For a particular solution of~\eqref{eq:nodespar}, the contribution from~\eqref{eq:hesspar} equals
\begin{equation}\label{eq:localcontpar}
    \frac{t-s}{t(t-1)s(s-1)}=\frac{(1-\zeta\mu)^3}{\zeta\mu(1-\zeta)(1-\mu)}.
\end{equation}
Let us compute the product over all solutions of~\eqref{eq:nodespar} of each factor in the right-hand side of~\eqref{eq:localcontpar}. To do that, we will multiply over all instances of the range $i=1,2,\dots,m-1$, $j=1,2,\dots,q-p$ and we will divide the exceeding terms that do not contribute according to the consideration given by each case.

For the factor $1-\zeta\mu$ in the numerator, let us observe that only multiples of $d_q$ can be obtained as integer combinations $iq+jm$, and each multiple $kd_p$ can be obtained $d_p$ times if $kd_p\not\equiv 0 \mod m$ and can be obtained $d_p-1$ times if $kd_p\equiv 0 \mod m$. After dividing by $d_p$, the product runs for $k=1,2,\dots, m_q(q-p)-1$ and we get that
\begin{equation}\label{eq:factonezetamu}
    \prod_{\mathrm{sols. to\eqref{eq:nodespar}}}(1-\zeta\mu)=
    \frac{\left[\displaystyle\prod_{l=1}^{m_q(q-p)-1}(1-\zeta_{m_q(q-p)}^{l})\right]^{d_q}}
    {\displaystyle\prod_{i=1}^{d_p-1}\left(1-\zeta_{m(q-p)}^{im_p(q-p)}\right) \cdot \prod_{j=1}^{q-p-1}\left(1-\zeta_{m_q(q-p)}^{jm_q}\right)}
    =\frac{\left[\displaystyle m_q(q-p)\right]^{d_q}}
    {\displaystyle d_p \cdot (q-p)},
\end{equation}
where $\zeta_{m_q(q-p)}$ is a primitive $m_q(q-p)$-th root of unity. The numerator has an excess of terms corrected by the second factor of the denominator corresponding to the multiples that appear only $d_p-1$ instead of $d_p$, and the first factor of the denominator correspond to elements $i,j$ such that $\zeta=1$ which do not contribute to our product. One can check that there are $d_q(m_q(q-p)-1)$ factors in the numerator and $[(q-p)-1+d_p+1]$ factors in the denominator, which account for twice the number of nodes of~$C'$.
Applying Lemma~\ref{lm:sineIdentity} yields the second equality in~\eqref{eq:factonezetamu}.

For the factor $\zeta\mu$ in the denominator we can use the same set of indices for the products in the equation. We get that
\begin{equation}\label{eq:factzetamu}
    \prod_{\mathrm{sols. to\eqref{eq:nodespar}}}(\zeta\mu)=
    \frac{\left[\displaystyle\prod_{l=1}^{m_q(q-p)-1}(\zeta_{m_q(q-p)}^{l})\right]^{d_q}}
    {\displaystyle\prod_{i=1}^{d_p-1}\left(\zeta_{m(q-p)}^{im_p(q-p)}\right) \cdot \prod_{j=1}^{q-p-1}\left(\zeta_{m_q(q-p)}^{jm_q}\right)}
    =\displaystyle \zeta_{m(q-p)}^{m(q-p)\left[\frac{m(q-p)-d_p-d_q-(q-p)+2}{2}\right]}=1,
\end{equation}
since~$m(q-p)-d_p-d_q-(q-p)+2\equiv0\mod2$ for all parities of~$m, p$ and~$q$.

For the factor $1-\zeta$ in the denominator the computation is analog to the one of $1-\zeta\mu$ by switching the roles of~$p$ and~$q$ due to the nature of the description in~\eqref{eq:zetapar} and~\eqref{eq:zetamupar}. Thus, we get that
\begin{equation}\label{eq:factonezeta}
    \prod_{\mathrm{sols. to\eqref{eq:nodespar}}}(1-\zeta)=
    \frac{\left[\displaystyle\prod_{l=1}^{m_p(q-p)-1}\left(1-\zeta_{m_p(q-p)}^{l}\right)\right]^{d_p}}
    {\displaystyle\prod_{i=1}^{d_q-1}\left(1-\zeta_{m(q-p)}^{im_q(q-p)}\right) \cdot \prod_{j=1}^{q-p-1}\left(1-\zeta_{m_p(q-p)}^{jm_p}\right)}
    =\frac{\left[\displaystyle m_p(q-p)\right]^{d_p}}
    {\displaystyle d_q \cdot (q-p)}.
\end{equation}
Lastly, for the factor $1-\mu$, for every instance of $i=1,2,\dots,m-1$, there are $q-p$ solutions for $j$ and we just need to correct for the solutions to $\zeta=1$ and $\zeta\mu=1$. Namely,
\begin{equation}\label{eq:factmu}
    \prod_{\mathrm{sols. to\eqref{eq:nodespar}}}(1-\mu)=
    \frac{\left[\displaystyle\prod_{i=1}^{m_-1}\left(1-\zeta_{m}^{i}\right)\right]^{q-p}}
    {\displaystyle\prod_{i=1}^{d_p-1}\left(1-\zeta_{m}^{i}\right) \cdot \prod_{i=1}^{d_q-1}\left(1-\zeta_{m}^{i}\right)}
    =\frac{\displaystyle m^{q-p}}{d_pd_q},
\end{equation}
by applying Lemma~\ref{lm:sineIdentity}.
The theorem follows from equations~\eqref{eq:welnodes} to~\eqref{eq:factmu} by considering terms up to squares in~$k$.
